Debugging of Markov Decision Processes (MDPs) Models

In model checking, a counterexample is considered as a valuable tool for debugging. In Probabilistic Model Checking (PMC), counterexample generation has a quantitative aspect. The counterexample in PMC is a set of paths in which a path formula holds, and their accumulative probability mass violates the probability threshold. However, understanding the counterexample is not an easy task. In this paper we address the task of counterexample analysis for Markov Decision Processes (MDPs). We propose an aided-diagnostic method for probabilistic counterexamples based on the notions of causality, responsibility and blame. Given a counterexample for a Probabilistic CTL (PCTL) formula that does not hold over an MDP model, this method guides the user to the most relevant parts of the model that led to the violation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{25}
\providecommand{\publicationstatus}{G. G\"ossler and O. Sokolsky (Eds.): 1st Workshop on Causal Reasoning for \\ Embedded and safety-critical Systems Technologies (CREST'16)\\
EPTCS 224, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.224.4}{10.4204/EPTCS.224.4}}
\pdfoutput=1

